Boundless: Generative Adversarial Networks for Image Extension

Image extension models have broad applications in image editing, computational photography and computer graphics. While image inpainting has been extensively studied in the literature, it is challenging to directly apply the state-of-the-art inpainting methods to image extension as they tend to generate blurry or repetitive pixels with inconsistent semantics. We introduce semantic conditioning to the discriminator of a generative adversarial network (GAN), and achieve strong results on image extension with coherent semantics and visually pleasing colors and textures. We also show promising results in extreme extensions, such as panorama generation.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
We have presented a novel model based on generative adversarial networks that perform well on image extension problems. Our results show the benefits of our architecture, training scheme, and our novel discriminator conditioning.However, our models have difficulties in completing humans, objects and animals. Improving the performance on such completions is a topic of further research. %

